RoomPlanner: Explicit Layout Planner for Easier LLM-Driven 3D Room Generation

In this paper, we propose RoomPlanner, the first fully automatic 3D room generation framework for painlessly creating realistic indoor scenes with only short text as input. Without any manual layout design or panoramic image guidance, our framework can generate explicit layout criteria for rational spatial placement. We begin by introducing a hierarchical structure of language-driven agent planners that can automatically parse short and ambiguous prompts into detailed scene descriptions. These descriptions include raw spatial and semantic attributes for each object and the background, which are then used to initialize 3D point clouds. To position objects within bounded environments, we implement two arrangement constraints that iteratively optimize spatial arrangements, ensuring a collision-free and accessible layout solution. In the final rendering stage, we propose a novel AnyReach Sampling strategy for camera trajectory, along with the Interval Timestep Flow Sampling (ITFS) strategy, to efficiently optimize the coarse 3D Gaussian scene representation. These approaches help reduce the total generation time to under 30 minutes. Extensive experiments demonstrate that our method can produce geometrically rational 3D indoor scenes, surpassing prior approaches in both rendering speed and visual quality while preserving editability. The code will be available soon.

==> history/0_abstract.tex <==
\begin{abstract}
Recent research in scene generation has produced relatively complete scenes; however, these scenes often exhibit limited complexity and lack diversity in object interactions. This limitation restricts the broader application of text-driven scene generation. In this paper, we propose RoomDreamer, an advanced text-to-3D scene generation model that generates high-quality 3D indoor scenes from textual descriptions. RoomDreamer leverages common-sense knowledge encoded in a large language model (LLM) to enhance its scene generation capabilities, utilizing a combination of a 2D diffusion model and 3D Gaussian Splatting (3DGS). This integration allows for the generation of diverse objects and coherent layouts without reliance on large-scale 3D asset datasets. Experimental results show that RoomDreamer generates higher-quality, more diverse, and realistic indoor scenes compared to state-of-the-art techniques, while utilizing fewer computational resources. The model and source code will be available shortly.
\end{abstract}

==> history/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

High-quality 3D indoor scene models are crucial for various industry applications such as scene simulation for embodied AI, gaming, film, and augmented/virtual reality (AR/VR)~\cite{Nießner13}. Traditionally, the creation of detailed 3D indoor scenes requires the expertise of professional designers, making it both an expensive and time-consuming process to scale data generation effectively.
\newline
Recent advancements in text-driven 3D generative models have significantly reduced the cost and complexity of scaling 3D indoor scene generation~\cite{Poole22}. These models can produce comprehensive 3D environments from simple textual prompts, thereby significantly enhancing design efficiency and increasing the diversity of indoor scenes~\cite{Zhang21}. Despite these advantages, many developers and designers still rely on traditional manual design methods that utilize large-scale 3D content libraries to build scenes~\cite{Savva19}. This raises a critical question: how can fully generative models become the most preferred approach for 3D indoor scene generation?
\newline
To fully realize the potential of generative models, three core criteria must be met: First, the models must ensure stable generation of high-quality scenes with detailed texture representation for excellent visual effects~\cite{Mildenhall20}. Second, they must guarantee both diversity and complexity in the generated scenes~\cite{Michel22}. Complexity is a crucial factor when evaluating generative versus manually designed scenes, while diversity prevents homogenization and supports adaptability for large-scale applications~\cite{Chang15}. Finally, the models must be capable of generating scenes that are not only visually coherent but also reflect the richness of real-world environments~\cite{Gao22}. Traditional scene generation methods often rely on large-scale 3D asset datasets, which can limit flexibility and scalability~\cite{Liu21}. In contrast, our generative model, RoomDreamer, uses powerful techniques like large language models (LLMs) and diffusion models to generate scenes from textual descriptions, offering more creative freedom and reducing reliance on existing 3D assets~\cite{Rombach22}. This shift in paradigm opens up new possibilities for applications such as gaming, virtual environments, and simulation-based training, where diverse and dynamic scenes are crucial~\cite{Yang23}.
\newline
At present, methods in the field of text-to-3D indoor scene generation can be categorized into two main types: semi-synthetic and semi-generative methods, which rely on synthetic material libraries, and fully generative paradigm methods~\cite{Chen21}. Although the semi-synthetic and semi-generative methods meet the core standards of high quality, they are based on sacrificing the richness of the scene, which is a major flaw for downstream large-scale applications~\cite{Sitzmann19}. In contrast, fully generative methods greatly increase the richness of the scene and are therefore receiving increasing attention~\cite{Park19}. These methods typically involve generating extensive 2D models and subsequently optimizing explicit 3D representations~\cite{Barron21}. Among these, GALA3D~\cite{Liu23} is a notable state-of-the-art (SOTA) method for text-to-3D indoor scene generation, known for its ability to meet the core criteria of diversity and stable high-quality scene generation.
\newline
However, existing state-of-the-art (SOTA) methods still exhibit limitations, particularly concerning downstream applications~\cite{Jun20}. A significant challenge is that current text-to-3D scene generation methods often struggle with generating scenes that are both diverse and complex, limiting their utility in dynamic and large-scale applications~\cite{Xu21}. 
% While there has been considerable research into enhancing scene generation with detailed object interactions and physical understanding, the integration of these elements with generative models remains limited~\cite{Zienkiewicz22}. 
Additionally, generating richer scenes still requires substantial computing resources and time, increasing the barrier for real-world applications to adopt text-to-3D scene generation~\cite{Chan22}. 
\newline
To address these challenges, we propose RoomDreamer, a novel method for generating high-quality 3D indoor scenes directly from textual descriptions. Our approach leverages a large language model to guide the layout and composition of the scene, while using diffusion models and 3D Gaussian splatting to create realistic 3D representations from multi-view images~\cite{Kerbl23}. By reducing reliance on large-scale 3D asset datasets and optimizing the generation process, RoomDreamer allows for more complex and diverse scene creation with lower computational costs and faster generation times~\cite{Ho20}. This method opens new possibilities for applications such as gaming, virtual environments, and simulation-based training, where rich, adaptable scenes are crucial~\cite{Zhang23}.


% To fully realize the potential of generative models, three core criteria must be met: First, the models must ensure stable generation of high-quality scenes with detailed texture representation for excellent visual effects. Second, they must guarantee both diversity and complexity in the generated scenes. Complexity is a crucial factor when evaluating generative versus manually designed scenes, while diversity prevents homogenization and supports adaptability for large-scale applications.  Finally, the generated content must incorporate physical realism and dynamic interaction logic. Traditional methods provide these physical bases and interaction requirements, which are currently lacking in generative paradigms. For applications such as games, films, and embodied simulations, the generated scenes must support dynamic and temporal interactions and provide relevant annotations and information.
% However, existing SOTA methods still exhibit limitations, particularly concerning downstream applications. A major defect that needs attention is that current text to 3D scene generation methods lack physical understanding of the scene objects. This defect has brought obstacles to downstream application focusing on interaction and simulation, such as embodied AI [5]. Although there is considerable research on physical understanding of scenes as a separate topic [6], integration with generative paradigms remains limited. Secondly, in order to generate richer scenes, it currently requires a lot of computing resources and time, which greatly increases the threshold for downstream applications to use Text to 3D scene generation. 
% \newline
% To address the above constraints and challenges, we propose DreamScene3D, a method designed to generate 3D indoor scenes that adhere to physical laws and incorporate physical understanding from simple text inputs. Our approach enables the creation of richer and more complex scenes with reduced time and cost. Specifically, we use a large language model and its common sense to guide the preliminary layout of indoor scenes. Then we use stable diffusion and depth estimation to lift multi-view images to 3D space. At the same time, we combine Gaussian splashing, which can provide smooth and continuous representations of point clouds, to generate more realistic 3D effects. Furthermore, we incorporate physical constraints, as detailed in PHYSCENE [7], to enhance the realism and coherence of the scenes. In addition, we used BLIP and a large language model to evaluate the physical information of all scene objects, offering crucial physical information for dynamic physical interactive expressions of downstream applications.


% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> history/2_RW.tex <==
\section{Related Work}
\label{sec:formatting}

%-------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{ICCV2025-Author-Kit-Feb/1.png} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Workflow Diagram of RoomDreamer.The input prompt integrates the OpenAI Large Language Model (LLM) through the LangChain framework to generate the room's Floor Plan and Wall Plan (the floor plan and wall structure of the room), Doorway Plan (the location of the door), Layout Plan (furniture layout, location and orientation) and Textural description of objects (furniture type, size). These textual descriptions are first converted into initial 3D Gaussian Splattings (3DGS) representation through the Text to 3D Generator, and then using a pre-trained stable diffusion model to guide 3D optimization. After empty room and furnitures generation, the furniture will be filtered through the Object Selector, leaving only semantically compliant, high-quality 3D assets. The filtered furniture will then be placed in the generated empty room based on the generated Layout Plan, and finally a complete 3D indoor scene will be generated.}
\label{fig:fig2}
\end{figure*}



%-------------------------------------------------------------------------
\subsection{Text-Driven 3D Objects Generation}
Current methodologies for text-driven 3D object generation are primarily categorized into two main approaches: direct utilization of 3D models for generation and lifting 2D expressions to 3D using the prior knowledge of 2D generation models. However, existing text-driven methods relying on combination of 3D models and diffusion model architectures~\cite{Rombach22} often struggle to achieve highly detailed or high-resolution outputs. In contrast, leveraging the prior knowledge in 2D generation models tends to yield superior results with more efficient resource utilization. Notably, recent advancements such as DreamFusion~\cite{Poole22}, which proposed supervising NeRF using score distillation sampling loss (SDS)~\cite{Poole22} of pre-trained 2D diffusion models, have popularized text-to-3D scene generation models based on 2D diffusion models~\cite{Michel22}. Since NeRF requires intensive computation and time-consuming rendering processes due to its reliance on volumetric ray sampling, Gaussian splatting 3D~\cite{Kerbl23} has emerged as a viable alternative, offering continuous and flexible 3D representation that facilitates efficient, high-quality rendering. The introduction of DreamGaussian~\cite{Tang23}, which optimizes 3D Gaussian splatting using score distillation sampling loss from pre-trained 2D diffusion models, has further underscored its potential, leading to continued research and optimization efforts in the 3D domain~\cite{Zhang23}. For instance, Lucidreamer~\cite{Li23} has integrated Interval Score Matching (ISM) to enhance Score Distillation Sampling (SDS), addressing its over-smoothing limitations.
% Current methodologies for text-driven 3D object generation are primarily categorized into two main approaches: direct utilization of 3D models for generation and lifting 2D expressions to 3D using the prior knowledge of 2D generation models. However, existing text-driven methods relying on combination of 3D models and diffusion model architectures ~\cite{} often struggle to achieve highly detailed or high-resolution outputs. In contrast, leveraging the prior knowledge in 2D generation models tends to yield superior results with more efficient resource utilization. Notably, recent advancements such as DreamFusion ~\cite{}, which proposed supervising NeRF using score distillation sampling loss ~\cite{} of pre-trained 2D diffusion models, have popularized text-to-3D scene generation models based on 2D diffusion models ~\cite{}. Since NeRF needs intensive computation and time-comsuming rendering process due to its reliance on volumetric ray sampling, Gaussian splatter 3D ~\cite{} has emerged as a viable alternative, offering continuous and flexible 3D representation that facilitates efficient, high-quality rendering. The introduction of DreamGaussian ~\cite{}, which optimizes 3D Gaussian splatter using score distillation sampling loss from pre-trained 2D diffusion models, has further underscored its potential, leading to continued research and optimization efforts in the 3D domain ~\cite{}. For instance, Lucidreamer ~\cite{} has integrated Interval Score Matching (ISM) to enhance Score Distillation Sampling (SDS), addressing its over-smoothing limitations.


%-------------------------------------------------------------------------
\subsection{Text-Driven 3D Scene Generation Evaluation}

For 3D object generation, there is already a complete set of evaluation criteria~\cite{Chang15}, but no unified evaluation framework exists for indoor 3D scene generation. Current evaluations of 3D scene models primarily rely on metrics such as Fréchet Inception Distance (FID)~\cite{Heusel17}, Kernel Inception Distance (KID)~\cite{Bińkowski18}, and Learned Perceptual Image Patch Similarity (LPIPS)~\cite{Zhang18} to assess visual quality. Others employ human-centric evaluations, including comprehensive questionnaires and Visual Question Answering (VQA)~\cite{Antol15}, to measure scene richness and complexity.
% For 3D object generation, there is already a complete set of evaluation criteria ~\cite{}, but there is no complete set of evaluation criteria for indoor 3D scene generation. At present, most of the evaluations of 3D scene models use indicators such as Fréchet Inception Distance (FID), Kernel Inception Distance (KID), Structural Content Assessment (SCA), Crop Knowledge Layer (CKL), Blind/Referenceless Image Spatial Quality Evaluator (BRISQUE), Naturalness Image Quality Evaluator (NIQE), Contrastive Language-Image Pretraining (CLIP), Peak Signal-to-Noise Ratio (PSNR), Structural Similarity Index (SSIM), Learned Perceptual Image Patch Similarity (LPIPS) to evaluate the authenticity or quality of the scene. Others use more comprehensive questionnaires and VQA ~\cite{} to evaluate the richness and complexity of generated scenes. 
% However, there is no set of metrics that can simultaneously detect the quality, complexity, authenticity and physical rationality of the scenes. Therefore, this paper proposes a relatively more complete set of evaluation metrics for Text-Driven 3D Scene Generation.

%-------------------------------------------------------------------------
\subsection{Text-Driven 3D Scene Generation}

% Current approaches to text-to-3D scene generation can be broadly classified into semi-generative-semi-synthetic and fully generative methods. Semi-generative-semi-synthetic methods refer to methods that incorporating existing high-definition 3D assets through retrieval methods ~\cite{Authors14} or rendering using texture datasets and established rendering tools like those available in Blender and Unity ~\cite{Authors14}. However, these methods that taking shortcuts often result in scenes lacking in diversity and richness, which cannot be solved under this framework, limiting their applicability in downstream applications. Consequently, there is a growing need for fully generative methods that can autonomously generate comprehensive scenes. 
Current approaches to text-to-3D scene generation can be broadly classified into semi-generative-semi-synthetic and fully generative methods. Semi-generative-semi-synthetic methods incorporate existing 3D assets through retrieval techniques~\cite{Savva19} or utilize texture datasets with rendering tools like Blender and Unity~\cite{Blender24}. However, these methods often produce scenes lacking diversity and richness, limiting their downstream applicability. Consequently, fully generative methods that autonomously synthesize scenes from textual prompts are gaining prominence.
\newline
Fully generative text-to-3D scene generation typically involves layout generation with spatial constraints to populate objects such as furniture and walls~\cite{Yang23}. GALA3D~\cite{Liu23}, which integrates supervised 3D Gaussian splatting optimization via SDS loss, represents a state-of-the-art approach in this domain. Despite advancements, current methodologies like GALA3D~\cite{Liu23} still struggle to achieve scene complexity comparable to real-world environments, posing challenges for practical applications.
% Fully generative text-to-3D scene generation typically involves designing or generating a basic layout and employing layout constraints to generate multiple objects such as furniture, walls, and floors. GALA3D ~\cite{Authors14}, which integrates supervised 3D Gaussian splatting optimization via score distillation sampling loss, represents a state-of-the-art approach in this domain. Despite advancements, current methodologies like GALA3D ~\cite{Authors14} still fall short in achieving scene complexity and quality comparable to real-world scenes, posing challenges for applications downstream.




\input{sec/table1}
% \input{sec/table2}


%-------------------------------------------------------------------------
% \subsection{Physical Understanding in 3D scene}
% Prior research on understanding physical properties in scenes has predominantly relied on dynamic scene observation [17, 18] or utilized 3D physics engines [19], both of which are resource-intensive and dependent on specific high-quality datasets. Recently, a novel approach [20] introduced a large language model capable of semantically screening candidate materials for objects without training. However, its physical understanding module remains disjointed from the scene generation process and relies heavily on datasets of high-quality scenes. In scene generation methods of semi-synthetic-semi-generative and manual scene generation, physical properties are often assigned to individual objects upon importing existing materials to facilitate integration into downstream applications. However, current fully generative 3D scene generation methods have yet to integrate physical understanding due to limitations in quality and stability of generated scene. To address this gap and facilitate seamless integration with downstream applications, there is a critical need to embed physical understanding directly into the generated 3D scenes. This necessity explains why many applications still prefer manually synthesized scenes despite higher costs and reduced richness. Hence, we propose a physical reasoning approach leveraging two large models, BLIP and ChatGPT-4, to bridge the gap between 3D scene generation and physical understanding, ensuring more cohesive integration into practical applications.

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> history/3_Method.tex <==
\section{Methodology}
\label{sec:formatting}



%-------------------------------------------------------------------------
\subsection{Overview}
Roomdreamer is an open promptable system based on 3D-Generate. It can create diverse, customized, and interactive indoor environments under the guidance of a large language model. As shown in Figure ~\ref{fig:fig2}, Roomdreamer employs a systematic approach to building scenes, utilizing a series of specialized modules: (1) Indoor environment : Formulate floor plans, build wall structures, and select appropriate materials for floors and walls. (2) Asset generation: Use Text-3D Module to produce materials based on the 3D asset descriptions provided by GPT-4. (3) Constraint-based layout design module: Arrange assets within the scene using spatial relationship constraints to ensure realistic indoor layouts.(4) Physical guidance: Provide physical understanding and descriptions of the scene to supervise all parts of the scene generation.

%-------------------------------------------------------------------------
\subsection{Text-to-3D Generation}
\noindent\textbf{Initialize 3D point-cloud shape} The raw 3DGS representation adopts the Gaussian densification scheme, providing good control over the total number of Gaussians. However, this strategy fails to constrain the distribution of Gaussian ellipsoids, resulting in numerous unused invisible Gaussians. It is also incapable of controlling Gaussian generation with a uniform regular shape, which shares similar covariances and normal vectors. As a comparison, we propose Adaptive Geometry Control for Gaussians, which achieves adaptive geometric control of Layout-guided Gaussians through distribution constraint and shape optimization.
Similar to ~\citep{Huang20, Low23}, given an initialized set of Gaussians, the distribution constraint can be implemented by a density distribution function:

\begin{equation}
  \frac{1}{\Vert \mathbf{p_i}- \mathbf{\zeta_i} \Vert} \sim \mathcal{\hat{N}} (\mu, \sigma^2),
  \label{eq:density}
\end{equation}

where $\mathbf{\zeta_i} = (x_i, y_i, z_i)$ is the center coordinate of the corresponding layout prior; $\Vert \mathbf{p_i}- \mathbf{\zeta_i} \Vert$ is the Euclidean distance between the Gaussian center and $\mathbf{\zeta_i}$; $\mu$ is the mean of the Gaussians' distributions; and $\sigma$ is the standard deviation. 
Both are changeable parameters.
Here, $\mathcal{\hat{N}}$ represents the folded normal distribution, with a truncation range from the layout center to the boundary.
We then sample Gaussians near the layouts' surface according to the distribution.

\noindent\textbf{Tansfer to 3D Gaussian Splatting} 3D Gaussian Splatting (3DGS) leverages the principles of Elliptical Weighted Average (EWA) volume splatting ~\cite{Zwicker01}  as the foundational technique for the efficient computation of 3D Gaussian kernel projections onto a 2D image plane. Building upon this, the method employs differentiable Gaussian splatting ~\cite{Kerbl23} to further refine the rendering process. This approach enables dynamic optimization of both the amount and the specific parameters of Gaussian kernels used for scene modeling. 

The optimized scene consists of millions of 3D Gaussians, each defined by a set of parameters: $\bm{x} \in \mathbb{R}^3$ for center position, $\bm{q} \in \mathbb{R}^4$ for the quaternion that represents the rotation, $\bm{s} \in \mathbb{R}^3$ for the scale of the Gaussian in each dimension, $\alpha \in [0,1]$ for the opacity, and 16 spherical harmonics (SH) coefficients for view dependent coloring. The covariance matrix of the Gaussian is calculated as follows:

\begin{equation}
    \bm{\Sigma} = R S S^T R^T
\end{equation}

where $R$ is the rotation matrix derived from the quaternion $q$ and $S$ is a diagonal scaling matrix constructed from the scale vector $s$. This formulation allows for the independent optimization of rotation and scaling, facilitating more flexible and precise control over the Gaussian's appearance in the rendered scene.

In the rendering process, the projection of a 3D Gaussian onto the 2D image plane is mathematically captured by transforming its covariance matrix:

\begin{equation}
    \bm{\Sigma'} = J W \Sigma \mathit{W}^T \mathit{J}^T,
\end{equation}

where $J$ is the Jacobian of the affine approximation of the projective transformation, and $W$ is the viewing transformation matrix that translates and rotates the 3D Gaussian from world coordinates into camera coordinates. This allows to evaluate the 2D color and opacity footprint of each projected Gaussian. The final pixel color $C$ is computed by blending $N$ 2D-Gaussians that contribute to this pixel, sorted in order of their depth


\subsection{Loss distillation control}

\noindent\textbf{IMSLoss}
We then introduce conditioned diffusion to optimize the global scene, generating interactions between multiple instances while adhering to the layout prior. Unlike single object generation, we use ControlNet~\cite{Zhang23ControlNet}  for compositional optimization, ensuring that the generated scene aligns with the layout. Concretely, we fine-tuned ControlNet to support rendering layouts from multiple viewpoints as input and generate 2D diffusion supervision with layout-text consistency. The gradients of SDS for scene parameters can be formulated as:
\begin{equation}
    \label{eq:native_ISM}
    \resizebox{0.89\linewidth}{!}{$\min_{\theta\in\Theta} \gL_{\mbox{\tiny ISM}}(\theta) :=   \E_{t,c} \left[\omega(t)||\vepsilon_\phi(\vx_{t}, t, y) - \vepsilon_\phi(\vx_s, s, \emptyset_{})||^2\right].$}
\end{equation}
Following~\cite{Poole22}, the gradient of ISM loss over $\theta$ is given by:
\begin{equation}
\label{eq:ISM_grad}
\resizebox{0.85\linewidth}{!}{$\nabla_{\theta} \gL_{\mbox{\tiny ISM}}(\theta) := \E_{t,c}\,[\omega(t) (\underbrace{\vepsilon_\phi(\vx_{t}, t, y_{}) - \vepsilon_\phi(\vx_s, s, \emptyset_{})}_{\text{ISM update direction}}) \frac{\partial\vg(\theta,c)}{\partial\theta}]\mbox{.}$}
\end{equation}


where $\delta$ is the condition input for the ControlNet, obtained by rendering the 2D images from the layouts. During the diffusion process, the instance-level and scene-level optimization share the same time step $\eta$ to ensure synchronous and collaborative learning. $t$ is the textual description of the whole scene encompassing multiple instances; $I$ is the rendered global scene from conditioned diffusion, and $G_{scene}$ denotes the parameters of scene Gaussians. 


Following previous works, Stable-diffusion3.0~\cite{StabilityAI23} is used for the text-to-3D pseudo-ground-truth to guide 3D asset render. The SDSLoss~\cite{Poole22} 
pioneers text-to-3D generation by seeking modes for the conditional post prior in the DDPM latent space. The SDS loss can be formulated as:
\begin{equation}
\label{eq:sds}
    \nabla_{\Theta} \mathcal{L}_\text{SDS} = \mathbb{E}_{t, p, \mathbf{\epsilon}}
    \left[
    w(t) (\epsilon_\phi(x_t; t, y) - \epsilon) 
    \frac {\partial x_t} {\partial {\Theta}}
    \right]
\end{equation}


\noindent\textbf{Multi-timestep Sampling} 
Flow Matching is a generative framework that learns a continuous transformation (flow) from a simple noise distribution \( p_0(x) \) to a target data distribution \( p_1(x) \), governed by the ordinary differential equation (ODE) 
\[
\frac{dx_t}{dt} = v_t(x_t),
\]
where \( x_t \) is the state at time \( t \in [0, 1] \), and \( v_t(x_t) \) is a learned velocity field. To implement this, the continuous flow is discretized into \( N \) time steps with step size \( \Delta t = \frac{1}{N} \), yielding discrete states \( x_0, x_1, \dots, x_N \). Starting from an initial noise sample \( x_0 \sim p_0(x) \), the state is iteratively updated using the Euler method:
\[
x_{k+1} = x_k + v_{t_k}(x_k) \cdot \Delta t,
\]
where \( t_k = k \Delta t \), and \( v_{t_k}(x_k) \) is the velocity field evaluated at step \( k \). This process repeats for \( k = 0, 1, \dots, N-1 \), generating the final state \( x_N \), which approximates the target distribution \( p_1(x) \). The velocity field \( v_t(x) \) is trained to minimize the discrepancy between the learned flow and the ideal conditional velocity field \( u_t(x_t \mid x_0, x_1) \), formulated as
\[
\mathcal{L}_{\text{FM}} = \mathbb{E}_{t, x_0, x_1} \left[ \| v_t(x_t) - u_t(x_t \mid x_0, x_1) \|^2 \right].
\]
% The deterministic nature of this update ensures reproducibility, while the adjustable step count \( N \) allows balancing computational efficiency and sample quality. Pseudocode for the multi-step denoising is provided below:

% \begin{verbatim}
% def generate_sample(v_t, x0, N):  
%     x, dt = x0, 1.0 / N  
%     for k in range(N):  
%         t = k * dt  
%         x += v_t(x, t) * dt  
%     return x  
% \end{verbatim}

This framework bypasses the iterative noise estimation of traditional diffusion models, achieving efficient generation through direct flow dynamics learning.


\noindent\textbf{Inversion with Stochastic Motion (ISM)}Given an input text prompt $\mathcal{P}$, our goal is to generate a set of multi-view latent variables $\{ \mathbf{z}_v \}_{v=1}^N$ in the diffusion model's latent space, where $N$ is the number of views (e.g., front, side, back). These latents, when decoded by a pretrained VAE, should produce 2D images $\{ \mathbf{x}_v \}_{v=1}^N$ that are both consistent with the text description and geometrically coherent for 3D reconstruction. The ISM framework optimizes latent variables through iterative noise injection and gradient-guided updates. Let $\mathbf{z}_t$ denote the latent variable at optimization step $t$, and $\mathbf{\epsilon}_\theta$ represent the diffusion model's noise prediction network.
% The process involves the following key steps:

% \begin{enumerate}
    % \item \textbf{Stochastic Noise Injection} \\
At each step $t$, we perturb the latent variable with Gaussian noise to explore the latent space:
\[
\mathbf{z}_t^{\text{noisy}} = (1 - \sigma_t) \mathbf{z}_{t-1} + \sigma_t \mathbf{\epsilon}, \quad \mathbf{\epsilon} \sim \mathcal{N}(0, \mathbf{I}),
\]
where $\sigma_t$ is the noise scale from the scheduler, and $\mathbf{\epsilon}$ is random noise.

% \item \textbf{Conditional Noise Prediction} \\
The noise prediction network $\mathbf{\epsilon}_\theta$ is conditioned on text embeddings $\mathbf{e}_{\text{text}}$:
\[
\mathbf{\epsilon}_\theta^{\text{cond}} = \mathbf{\epsilon}_\theta\left(\mathbf{z}_t^{\text{noisy}}, t, \mathbf{e}_{\text{text}}\right),
\]
\[
\mathbf{\epsilon}_\theta^{\text{uncond}} = \mathbf{\epsilon}_\theta\left(\mathbf{z}_t^{\text{noisy}}, t, \mathbf{e}_{\text{null}}\right),
\]
where $\mathbf{e}_{\text{null}}$ represents null-text embeddings for unconditional prediction.

% \item \textbf{Classifier-Free Guidance (CFG)} \\
To enhance text alignment, the final noise prediction combines conditional and unconditional outputs:
\[
\mathbf{\epsilon}_\theta = \mathbf{\epsilon}_\theta^{\text{uncond}} + s \cdot \left( \mathbf{\epsilon}_\theta^{\text{cond}} - \mathbf{\epsilon}_\theta^{\text{uncond}} \right),
\]
where $s$ is the guidance scale (hyperparameter).

% \item \textbf{Gradient Computation} \\
We compute the gradient of the latent variable to minimize the deviation from the target distribution:
\[
\nabla_{\mathbf{z}_t} \mathcal{L} = \sigma_t \left( \mathbf{\epsilon}_\theta - \mathbf{\epsilon} + \mathbf{z}_t^{\text{noisy}} \right),
\]
where $\mathcal{L}$ is the implicit loss function derived from the diffusion objective.

\textbf{Latent Variable Update} \\
The latent variable is updated using gradient descent with learning rate $\eta$:
\[
\mathbf{z}_{t+1} = \mathbf{z}_t^{\text{noisy}} - \eta \cdot \nabla_{\mathbf{z}_t} \mathcal{L}.
\]
% \end{enumerate}

To ensure geometric coherence across views, we enforce consistency between predicted depths $\mathbf{d}_v$ and latent gradients. Let $\mathcal{M}_v$ denote a depth-based mask for view $v$, normalized to $[0, 1]$. The gradient is masked to focus on geometrically stable regions:
\[
\nabla_{\mathbf{z}_t} \mathcal{L}_{\text{3D}} = \mathcal{M}_v \odot \nabla_{\mathbf{z}_t} \mathcal{L},
\]
where $\odot$ is element-wise multiplication. This ensures that updates prioritize regions with reliable depth estimates.

% The ISM algorithm proceeds as follows: \\
% \textbf{Input}: Text prompt $\mathcal{P}$, initial latent $\mathbf{z}_0$, scheduler $\{\sigma_t\}_{t=1}^T$. \\
% \textbf{Output}: Optimized multi-view latents $\{\mathbf{z}_v\}_{v=1}^N$.

% \begin{enumerate}
%     \item Encode text into embeddings $\mathbf{e}_{\text{text}}$.
%     \item For each view $v \in \{1, \dots, N\}$:
%     \begin{enumerate}
%         \item \textbf{For} $t = 1$ to $T$:
%         \begin{enumerate}
%             \item Inject noise: $\mathbf{z}_t^{\text{noisy}} = (1 - \sigma_t)\mathbf{z}_{t-1} + \sigma_t \mathbf{\epsilon}$.
%             \item Predict noise $\mathbf{\epsilon}_\theta$ via CFG.
%             \item Compute gradient $\nabla_{\mathbf{z}_t} \mathcal{L}$.
%             \item Apply depth-based masking: $\nabla_{\mathbf{z}_t} \mathcal{L}_{\text{3D}}$.
%             \item Update latent: $\mathbf{z}_t = \mathbf{z}_t^{\text{noisy}} - \eta \nabla_{\mathbf{z}_t} \mathcal{L}_{\text{3D}}$.
%         \end{enumerate}
%         \item Decode $\mathbf{z}_T$ to image $\mathbf{x}_v$.
%     \end{enumerate}
%     \item Aggregate latents $\{\mathbf{z}_v\}$ for 3D reconstruction.
% \end{enumerate}

This methodology bridges diffusion-based 2D generation and 3D reconstruction, enabling high-fidelity text-to-3D generations. Key contributions include stochastic exploration to prevent local optima traps, gradient-guided refinement to align 2D generations with 3D geometric priors, and multi-view harmonization to ensure consistency across views.


\noindent\textbf{FMSLoss}
We then introduce stable-diffusion3.0 ~\cite{StabilityAI23} to optimize the global scene, 
% 与以往基于DDIM的其他版本的stable-diffusion\cite{[],[]}不同，stable-diffusion采用FlowMatching作为scheduler来对噪声进行采样。这意味着以往在DDIM上使用的SDSLoss需要进行转换才能进行使用

\begin{equation}
\label{eq:zt}
z_t = (1 - t) x_0 + t \epsilon
\end{equation}

With some simple computation, we cloud transform Eq.~\eqref{eq:zt} as:

\begin{equation}
\label{eq:zt_noise}
z_t = x_0 + t \underbrace{( \epsilon - x_0)}_{\text{noise}}
\end{equation}

Then, combining Eq.~\eqref{eq:sds} and Eq.~\eqref{eq:zt_noise}, we cloud get the FMS loss can be formulated as:
\begin{equation}
    % \small
    \nabla_{\Theta} \mathcal{L}_\text{FMS} = \mathbb{E}_{t, p, \mathbf{\epsilon}}
    \left[
    w(t) (\epsilon_\phi(z_t; t, y) - \underbrace{(\epsilon - x_0)}_{\text{noise}}) 
    \frac {\partial x_t} {\partial {\Theta}}
    \right]
\end{equation}


\noindent\textbf{IFMSLoss}
we cloud get the IFMS loss can be formulated as:
\begin{equation}
    % \small
    \nabla_{\Theta} \mathcal{L}_\text{FMs}=\mathbb{E}_{t, p, \mathbf{\epsilon}}
    \left[
    w(t)(\epsilon_\phi(z_t; t, y)-(\epsilon_\phi(z_t; S, \emptyset_{} )) 
    \frac {\partial x_t}{\partial {\Theta}}
    \right]
\end{equation}

\subsection{Physical Guidance and Constraint}
\label{sec:constraints}

\textbf{Holodeck-Based Physics-Aware Layout Generation}\\
As shown in the fourth module of Figure~\ref{fig:fig2}, we implement Holodeck's constraint-based framework~\cite{holodeck2023} for object positioning and orientation determination. Following Holodeck's methodology~\cite{holodeck2023}, we adopt its spatial constraint engine to process qualitative relationships (e.g., ``coffee table adjacent to sofa'') generated by LLMs, rather than directly predicting numerical coordinates as in prior LLM-based approaches~\cite{feng2023layoutgpt}. This strategy inherits Holodeck's robustness against boundary violations and collision errors in complex scene composition.
\newline
\textbf{Holodeck Constraint Taxonomy Implementation}\\
We strictly adhere to Holodeck's predefined constraint system~\cite{holodeck2023}, which categorizes spatial rules into five classes: 
\begin{itemize}
    \item \textit{Global}: Edge/middle alignment
    \item \textit{Proximity}: Near/far thresholds
    \item \textit{Positional}: Front/side/vertical placement
    \item \textit{Alignment}: Centroid matching
    \item \textit{Orientation}: Facing direction
\end{itemize}
These constraints are organized into a scene graph following Holodeck's specification. The framework maintains Holodeck's original constraint hierarchy: soft constraints permit controlled violations through weighted optimization, while hard constraints strictly enforce collision prevention and boundary compliance.
\newline
\textbf{Holodeck Constraint Resolution Protocol}\\
We reproduce Holodeck's mathematical formalization~\cite{holodeck2023} that converts spatial relationships to geometric conditions:
\begin{equation}
    |x_i - x_j| < \epsilon \quad \text{(centroid alignment)}
\end{equation}
The placement pipeline follows Holodeck's standard workflow:
\begin{enumerate}
    \item LLM-based anchor object selection (e.g., bed in bedrooms)
    \item Depth-First Search (DFS)
    % \footnote{Holodeck supports alternative solvers like MILP; we use DFS for consistency with its baseline implementation.} for dependent object placement
\end{enumerate}



% %
% \subsection{Physical Guidance and Constraint}
% % 我们遵循着GPT4提供的layout指导，对xxx进行生成, 我们根据实际场景希望，可以给出，{x,y,z}
% % 参考holodeck，完成 XXXX
% \smallbreak
% \noindent The \textbf{LLM-based Physic imformation Guidance}, illustrated in the fourth panel of Figure~\ref{fig: pipeline}, generates the positioning and orientation of objects. Previous work \cite{feng2023layoutgpt} shows LLM can directly provide the absolute value of the object's bounding box. However, when attempting to place a diverse lot of assets within environments, this method frequently leads to out-of-boundary errors and object collisions. To address this, instead of letting LLM directly operate on numerical values, we propose a novel constraint-based approach that employs LLM to generate spatial relations between the objects, e.g., ``coffee table, in front of, sofa'', and optimize the layout based on the constraints. Given the probabilistic nature of LLMs.

% \smallbreak
% \noindent The \textbf{Constraint-based Layout Design Module}, illustrated in the fourth panel of Figure~\ref{fig: pipeline}, generates the positioning and orientation of objects. Previous work \cite{feng2023layoutgpt} shows LLM can directly provide the absolute value of the object's bounding box. However, when attempting to place a diverse lot of assets within environments, this method frequently leads to out-of-boundary errors and object collisions. To address this, instead of letting LLM directly operate on numerical values, we propose a novel constraint-based approach that employs LLM to generate spatial relations between the objects, e.g., ``coffee table, in front of, sofa'', and optimize the layout based on the constraints. Given the probabilistic nature of LLMs.

% \smallbreak
% \noindent \textbf{Spatial Relational Constraints.} We predefined ten types of constraints, organized into five categories: (1) Global: \textit{edge}, \textit{middle}; (2) Distance: \textit{near}, \textit{far}; (3) Position: \textit{in front of}, \textit{side of}, \textit{above}, \textit{on top of}; (4) Alignment: \textit{center aligned} and (5) Rotation: \textit{face to}. LLM selects a subset of constraints for each object, forming a scene graph for the room (examples shown in Figure \ref{fig: constraints}). Those constraints are treated softly, allowing for certain violations when finding a layout to satisfy all constraints is not feasible. Besides those soft constraints, we enforce hard constraints to prevent object collisions and ensure that all objects are within the room's boundaries. 
% \smallbreak
% \noindent \textit{Constraint Satisfaction.} We first reformulate the spatial relational constraints defined above into mathematical conditions (e.g., two objects are center-aligned if they share the same $x$ or $y$ coordinate). To find layouts that satisfy constraints sampled by LLMs, we adopt an optimization algorithm to place objects autoregressively. The algorithm first uses LLM to identify an anchor object and then explores placements for the anchor object. Subsequently, it employs Depth-First-Search (DFS)\footnote{Given the linear nature of constraints, a Mixed Integer Linear Programming (MILP) solver can also be employed. While we assume the DFS solver in our experiments, we analyze the MILP solver in the supplements.} to find valid placements for the remaining objects. A placement is only valid if all the hard constraints are satisfied.

% For example, in Figure \ref{fig: constraints}, \textit{bed} is selected as the anchor object in the \textit{bedroom}, and the \textit{nightstands} are placed subsequently. The algorithm is executed for a fixed time (30 seconds) to get multiple candidate layouts and return the one that satisfies the most total constraints. We verify the effectiveness of our constraint-based layout in Sec \ref{sec: layout ablation}.

% \textbf{\ani{Slightly off heading for this content. When I read Scale, I thought about the size of rooms / environments with many rooms etc. Perhaps you can refer to this as sampling, and then give some details on how you sample, and how this can lead to an exponential generation of envs.}
% }
%\medbreak

% %-------------------------------------------------------------------------
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{ICCV2025-Author-Kit-Feb/2.jpg} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{.}
% \label{fig3}
% \end{figure*}


%-------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{ICCV2025-Author-Kit-Feb/3.jpg} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Multi-View Visualization of Individual Rooms Generated by RoomDreamer.}
\label{fig:fig4}
\end{figure*}




==> history/4_Experiments.tex <==
\section{Experiments}
\label{sec:formatting}
%-------------------------------------------------------------------------
\noindent \textbf{}% Our method is implemented in PyTorch~\cite{paszke2019pytorch}, based on ThreeStudio~\cite{threestudio2023}. The 3D diffusion models used in our method are Shap-E~\cite{jun2023shap} and MDM~\cite{tevet2022mdm}, and we load the Shap-E model finetuned on Objaverse~\cite{deitke2023objaverse} in Cap3D~\cite{luo2023scalable}.
For the 2D diffusion model, we use \emph{stable-diffusion 3.0}~\cite{StabilityAI23}, with a guidance scale of $100$. The timestamps we use are uniformly sampled from 0.02 to 0.98 before 500 iterations, and change to 0.02 to 0.55 after 500 iterations. 
For the 3D Gaussians, the learning rates of opacity $\alpha$ and position $\mu$ are $10^{-2}$ and $5 \times 10^{-5}$. The color $c$ of the 3d Gaussians is represented by the sh coefficient, with the degree set to 0 and the learning rate set to $1.25 \times 10^{-2}$. The covariance of the 3D Gaussians is converted into scaling and rotation for optimization, with learning rates of $10^{-3}$  and $10^{-2}$, respectively.
The radius of the camera we use for rendering is from 1.5 to 4.0, with the azimuth in the range of -180 to 180 degrees and the elevation in the range of -10 to 60 degrees.
The total training iterations are $1200$. All our experiments can be completed within 15 minutes on a single RTX 3090 with a batch size of 4.
The resolution we use for rendering is 1024 $\times$ 1024, which is scaled to 512 $\times$ 512 when optimizing using the 2D diffusion model. We can render in real time at 512 $\times$ 512 resolution. And all our code will be released.
To comprehensively evaluate the effectiveness of our proposed text-to-3D scene generation model based on 3D Gaussian Splatting and Stable Diffusion, we designed a series of experiments. 


% %-------------------------------------------------------------------------
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{ICCV2025-Author-Kit-Feb/4.jpg} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{.}
% \label{fig5}
% \end{figure*}


%-------------------------------------------------------------------------
\subsection{Quantitative Evaluation}
As shown in Table\ref{tab:Unconditioned Scene Synthesis}, we conducted quantitative evaluations using the T3 benchmark, which provides a rich set of text descriptions and corresponding 3D models for assessing the performance of generating both single objects and multiple objects. 
% We employed commonly used evaluation metrics such as Chamfer Distance (CD) to measure surface distance, Earth Mover's Distance (EMD) to evaluate point cloud distribution differences, and Fréchet Inception Distance (FID) to assess feature space distribution differences. 
Our method was compared against state-of-the-art text-to-3D methods, and the results are presented in tables and charts, highlighting the advantages of our approach in terms of generation quality and diversity.
Furthermore, we analyzed the computational efficiency of our method by recording training and inference times and comparing them with those of other state-of-the-art methods. This analysis demonstrated the efficiency of our approach, particularly in terms of resource utilization and scalability. 



%-------------------------------------------------------------------------
\subsection{Qualitative Evaluation}
In addition to quantitative evaluation, we performed qualitative assessments to showcase the practical capabilities of our method. As shown in Figure ~\ref{fig:fig5} and Figure ~\ref{fig:fig4}, we generated 3D assets of individual furniture and complete scenes, providing rendered images from various viewpoints to visually demonstrate the quality and detail of the outputs. 
% To further validate the usability of the generated scenes, we conducted a user study where participants rated the results based on realism, diversity, and plausibility. Additionally, we selected several representative cases for in-depth analysis, illustrating our method's ability to handle complex scenes and intricate details, such as object interactions and spatial coherence.



% %-------------------------------------------------------------------------
% \subsection{Ablation Studies}
% To understand the contribution of each component in our pipeline, we conducted ablation studies. Specifically, we examined the impact of the 3D Gaussian Splatting module by comparing results with and without its inclusion. We also explored the influence of different versions of the Stable Diffusion model on generation quality and tested various loss functions to identify their effects on the final output. These experiments provided insights into the importance of each module and guided further optimization of the model.


% \noindent \textbf{Constraint-based layout is more reliable.}
% Table \ref{tab:placement_abalation} reports the Mean Reciprocal Rank of different layout design methods. holodeck's constraint-based approach outperforms the other methods significantly on \textit{bathroom}, \textit{bedroom} and \textit{living room}. \textsc{Constraint} and \textsc{Edge} perform similarly on \textit{kitchen}, where it is common to align most objects against walls. The \textsc{Absolute} method performs no better than \textsc{Random} due to its tendency to create scenes with collision and boundary errors (see examples in the supplement), typically rated poorly by humans. These results endorse spatial relational constraints as a viable strategy for generating scenes that adhere to commonsense logic.


==> history/5_Conclusion.tex <==
\section{Conclusion and Limitation}
In this work, we introduced RoomDreamer, a novel framework for generating high-quality 3D indoor scenes directly from textual descriptions. By leveraging the strengths of large language models (LLMs), diffusion models, and 3D Gaussian splatting, RoomDreamer addresses the critical challenges of diversity, complexity, and computational efficiency in text-to-3D scene generation. RoomDreamer demonstrates that fully generative models can meet the core criteria of high-quality texture representation, scene diversity, and complexity, making them a viable alternative to traditional manual design methods. By integrating LLMs for scene layout guidance and diffusion models for realistic 3D representation, our method achieves a balance between visual fidelity and computational efficiency. Experimental results show that RoomDreamer outperforms existing state-of-the-art methods in generating diverse and complex scenes while requiring fewer computational resources. This advancement paves the way for broader adoption of generative models in industries that demand scalable and dynamic 3D content creation.
\newline
Despite its promising results, RoomDreamer has certain limitations that warrant further investigation. While RoomDreamer incorporates 3D Gaussian splatting for realistic representations, it does not fully simulate physical properties such as object collisions, material interactions, or lighting effects. Integrating advanced physical simulation techniques could further enhance the realism and usability of generated scenes for applications like embodied AI training and virtual environments. Finally, the current evaluation of RoomDreamer focuses on indoor scenes, and its performance in generating outdoor or hybrid environments remains unexplored. Extending the framework to handle diverse scene types and scales is an important direction for future work.
\newline
In conclusion, RoomDreamer represents a significant step forward in text-to-3D scene generation, addressing key challenges in diversity, complexity, and computational efficiency. However, overcoming the aforementioned limitations will be crucial for unlocking the full potential of generative models in real-world applications. Future research could explore integrating advanced physical simulations, improving robustness to textual inputs, and extending the framework to support a wider range of environments and use cases.


==> history/6_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> history/math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts, bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\x}{\vx}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}
\def\vtheta{{\bm{\theta}}}
\def\vphi{{\bm{\phi}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\veta{{\bm{\eta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution


\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
    #1\;\delimsize\|\;#2%
}
\newcommand{\kl}{D_{\mathrm{KL}}\infdivx}

\newcommand{\dm}{\mathrm{d}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% reference commands
\newcommand{\reff}[1]{Fig.~\ref{fig:#1}}
\newcommand{\reft}[1]{Tab.~\ref{table:#1}}
\newcommand{\refe}[1]{Eqn.~(\ref{eqn:#1})}
\newcommand{\refs}[1]{Sec.~\ref{sec:#1}}



\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> history/sec/0_abstract.tex <==
\begin{abstract}

% Recent research in scene generation has produced relatively complete scenes. However, these kinds of methods rely on material repositories, which are often constrained in terms of diversity and fail to facilitate interactions between objects.

In this paper, we propose \textit{\Ourmodel}, the first fully automatic 3D room generation framework for painlessly creating realistic indoor scenes with only short text as input. Without any manual layout design or panoramic image guidance, our framework can generate explicit layout criteria for rational spatial placement. We begin by introducing a hierarchical structure of language-driven agent planners that can automatically parse short and ambiguous prompts into detailed scene descriptions. These descriptions include raw spatial and semantic attributes for each object and the background, which are then used to initialize 3D point clouds. To position objects within bounded environments, we implement two arrangement constraints that iteratively optimize spatial arrangements, ensuring a collision-free and accessible layout solution.
In the final rendering stage, we propose a novel AnyReach  Sampling strategy for camera trajectory, along with the  Interval Timestep Flow Sampling (ITFS) strategy, to efficiently optimize the coarse 3D Gaussian scene representation. These approaches help reduce the total generation time to under 30 minutes. % change to 30
Extensive experiments demonstrate that our method can produce geometrically rational 3D indoor scenes, surpassing prior approaches in both rendering speed and visual quality while preserving editability. The code will be available soon.%at [URL].
  
\end{abstract}

%Specifically, our high-level planner interprets user input prompts into descriptions that select initial objects aligned with the semantics of the required scene. The low-level planner can ground detailed descriptions, including raw spatial and semantic attributes for each object asset and the background.


==> history/sec/1_intro.tex <==
\section{Introduction}

Text-to-3D scene generation aims to convert textual descriptions into 3D environments. Designed to lower costs and reduce the required expertise, this paradigm is conducive to various downstream applications, such as embodied AI~\cite{chen2024urdformer,embodiedscan}, gaming~\cite{wonderworld}, filmmaking, and augmented / virtual reality~\cite{Real-time3D}. Benefitting from the remarkable success of generation models~\cite{diffusion, ddim} and implicit neural representation~\cite{nerf,3DGS}, numerous methods have emerged to address the challenges of text-to-3D object generation, achieving significant milestones. However, directly transitioning from generating 3D assets to creating complete scenes is not a trivial task. This is partly due to the fact that layout information requires additional context and human effort. Based on the extracted layout sources, existing 3D scene generation methods can be broadly classified into two categories: \textbf{I.}~\emph{Visual-guided}, and \textbf{II.}~\emph{Rule-based} methods. 

Visual-guided methods rely on extracting implicit spatial information from visual representations, \eg~multi-view RGB or panorama images. Methods in this category typically adopt a two-stage generation framework, where image generation serves as an intermediate process, followed by an implicit neural representation network that renders a 3D scene from previously generated images. Some methods~\cite{director3d, scene4u} treat objects and backgrounds as an indivisible whole as input for the implicit rendering network. As a result, these continuous representations produced by these methods lack object-level decoupling, which significantly restricts practical use. These kinds of approaches can also lead to foggy or distorted geometry, as shown in~\cref{fig:teaser} (b). %Methods like SceneWiz3D~\cite{Zhang_2024_CVPR} enable object-level manipulation by introducing a hybrid 3D representation that combines explicit representations for objects with implicit representations for scenes. 
Instead of being directly constrained, the layout configuration is learned from a text-to-image generation model, which is optimized by aligning the generated images with the input text using a similarity score. Thus, the optimization of the scene configuration is constrained by the capabilities of the image generation model, making it difficult to directly control the layout through textual descriptions. %Additionally, this process relies on human-designed layouts for initialization and requires manual processing for object arrangement. 

Rule-based methods, on the other hand, explicitly utilize predefined rules based on physical relationships and constraints to create layout information of 3D environments.
Early methods~\cite{dreamscene,GALA3D,setthescene,Text2Room} depend on manually crafted prompt templates or human-designed layouts for initialization, which helps generate physically plausible scenes. This procedure relies on specialized expert knowledge and typically involves a tedious trial-and-error process to refine predefined spatial attributes of objects,~\eg~ position, size, and rotation~\etc. This human-in-the-loop paradigm increases the demand for human labor while also undermining the end-to-end training process.

\begin{figure*}
  \centering
  \includegraphics[width=1.0\textwidth]{figures/teaser.pdf}
  \caption{Compared to previous methods,~\ie visual-guided method Pano2Room~\cite{pu2024pano2room} and rule-based method DreamScene~\cite{dreamscene}, our approach effectively generates indoor scenes characterized by (a) more realism, (b) smoother mesh structures, and (c) support for a diverse array of editions, including operations such as rotation, translation, importing/deleting 3D assets, and style variations. }
  \label{fig:teaser}
\end{figure*}

On a separate line of research and to reduce human effort in layout design, data-driven approaches treat scene synthesis as a 3D asset arrangement task within a bounded environment. These methods add objects sequentially using an order prior with a forest structure ~\cite{sun2024forest2seq} or simultaneously through conditional score evaluation ~\cite{maillard2024debara}. Recently, Large Language Models (LLMs) have been introduced to automate the creation of 3D scenes~\cite{holodeck2023, yang2024llplace, Sun_2025_CVPR}. LLMs can directly translate unstructured language into structured spatial representations, which reduces dependence on rigid templates. However, their reliance on existing 3D assets limits the versatility and flexibility required to generate diverse and innovative scenes.

In this paper, we present \textbf{\Ourmodel}, which combines the advances of visual-guided and rule-based models. Unlike previous approaches, our method enables automatic generation of differentiable 3D scenes and layout constraints given only short textual prompts. Our framework adopts a `Reasoning-Grounding, Arrangement, and Optimization' pipeline to break down the complex 3D scene generation task into controllable and scalable subtasks. In the reasoning and grounding stage, our hierarchical LLM-driven agent planners can parse short user prompts into executable long-term descriptions. Specifically, our high-level LLM agent produces textual descriptions that select the initial target scene and objects that satisfy the contextual semantics. The low-level LLM agent generates fine-grained grounding descriptions that infer object and background scales, along with layout rules that match real-world dimensions. These explicit physical constraints also ensure that the generated 3D scenes meet the interaction requirements.

After obtaining the initial scene description from the LLM agents, we utilize a text-to-3D object generator~\cite{shap-e} to create 3D assets represented as point clouds. To assign initial object assets into the scene, we then employ interactive optimization to update the layout design by verifying whether the generated layout meets our constraints. To improve the rationality of the indoor scene, we first apply collision constraints to detect overlaps between objects. Additionally, we introduce a reachability constraint to assess path viability between entry points and target assets, supporting dynamic asset placement through closed-loop optimization. The generated scenes remain fully editable at both the object and global levels, allowing for reposition, insertion, deletion, and style transfer, as shown in~\cref{fig:teaser} (c). 

For photorealistic rendering, we introduce a module that integrates Interval Timestep Flow Sampling (ITFS) with reflection flow matching and hierarchical multi-timestep sampling. By leveraging a 2D diffusion prior and detailed scene descriptions from LLM agents, this module generates continuous 3D representations that exhibit a realistic appearance and rich semantics. We also propose the AnyReach camera trajectory sampling strategy that can optimize both object-centric and global views within a single rendering pass. Consequently, our pipeline produces high-fidelity scenes in a single optimization stage, reducing the overall runtime by nearly 2× compared to prior work.



==> history/sec/2_related.tex <==
\section{Related Work}
\label{rw}

\subsection{Text-to-3D Object Generation}
Existing 3D scene generation methods can be broadly classified into two categories: \textbf{I.}~\emph{Visual-Guided}, and \textbf{II.}~\emph{Direct regression} methods. 
Visual-Guided methods~\cite{prolificdreamer,luciddreamer,Trellis} rely on pretrained 2D diffusion models, which can lead to error accumulation during the subsequent image-to-3D conversion process. While MagicTailor~\cite{magictailor} addresses the issue of semantic pollution in the text-to-image stage, the resulting continuous representations still struggle with object-level decoupling. Direct regression methods~\cite{point-e,shap-e} focus on generating 3D assets directly from input text. Although 3D object generation has made significant advancements, directly applying a similar philosophy to solve 3D scene generation is still very challenging. Due to the lack of high-quality text-to-3D scene datasets, it hinders the ability to implement a feed-forward network directly. Furthermore, incorporating layout information adds an additional layer of complexity to the scene synthesis process.

\subsection{LLM driven 3D Scene Generation}
As discussed in \textsection Introduction, rule-based methods can utilize explicit layout information to generate accurate and diverse 3D layouts. However, designing an effortless mechanism for layout arrangement remains an open question in 3D scene synthesis. With the reasoning capabilities of LLMs, works such as LayoutGPT~\cite{layoutgpt} and SceneTeller~\cite{sceneteller} can generate visual layouts and place existing 3D assets for scene synthesis. However, because of the single-step planning strategy, their output often exhibits physical implausibilities,~\eg~floating objects or intersecting geometries. Additionally, they tend to perform suboptimally in complex scenes with numerous objects, mainly due to the absence of spatial constraints. %\XL{Our close-loop arrangement mechanism can solve this issue.}

On the other hand, LLM-driven frameworks aim to reduce human effort in the 3D layout arrangement task. To improve layout rationality, recent reinforcement learning-based methods utilize constraint solvers to enhance physical validity. Holodeck~\cite{holodeck2023} and its extensions~\cite{yang2024llplace,Sun_2025_CVPR} translate relational phrases into geometric constraints, which are optimized using gradient-based methods to eliminate collisions.  Diffuscene~\cite{diffuscene} and Physcene~\cite{physcene} incorporate physics engines to simulate object dynamics, iteratively adjusting parameters derived from LLMs to ensure stability. Despite advances in realism, their reliance on existing 3D assets limits the versatility and flexibility needed for generating diverse and innovative scenes. Beyond these layout arrangement approaches, our model provides a fully automated pipeline for generating complete and controllable 3D scenes, including individual decoupling objects.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 润色prompt
% The above text is refined to improve coherence and conform to ICML/NIPS/ICLR writing styles, ensuring that the logic is consistent with the original text, and that no extras are added and no inappropriate content is added. Check for grammatical, semantic, and logical errors and fix them. Be careful to make the touched-up text as consistent as possible with the style of the native writers, and avoid the phenomenon of Chinese English.

==> history/sec/3_method.tex <==
\section{Methodology}
\label{method}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.42\textwidth]{figures/fig3.pdf}
  \caption{~\Ourmodel~follows a `Reasoning-Grounding, Arrangement, and Optimization' pipeline, decomposing the complex 3D scene generation task into scalable subtasks. }
  \label{fig:pipeline}
\end{figure}

\Ourmodel~is a fully automated pipeline designed to generate complete, complex, and controllable 3D indoor scenes from concise user prompts. As shown in~\cref{fig:pipeline}, our framework comprises three main components. We begin by introducing a hierarchical LLM-driven planner that reasons and grounds the target room type based on the user prompt. It produces detailed textual descriptions ${y_i}{(i=1,...,N)}$ for each asset and a scene layout configuration $y_\text{scene}$. Next, we create the initial 3D point cloud for each asset using a text-to-3D object generator~\cite{shap-e} with $y_i$ as input. Meanwhile, a layout planner computes the optimal sizes and poses for the assets, generating a complete scene map that includes object coordinates, orientations, physical properties, and style descriptions. The assets are then positioned within the coordinate system of the room, according to pose specifications. Finally, we employ an Interval Timestep Flow Sampling with a novel camera sampling strategy to perform single-stage scene optimization, yielding results with realistic visuals and high 3D consistency.


\begin{algorithm}[t]
\caption{~\Ourmodel~Framework}
\label{alg:framework}
\begin{algorithmic}[1]
\State \textbf{Input}: short‑prompt description $\{\mathbf{I}\}$
\State \textbf{Output}: 3D room scene $\mathbf{Scene}^{\star}$

\State \textcolor{gray}{// High‑Level Reasoning}
\State $(\mathcal{O},\mathcal{S}) \gets \textsc{LLMParse}(\mathbf{I})$

\State \textcolor{gray}{// Low‑Level Grounding}
\State $\mathcal{P} \gets \textsc{InitPointCloud}(\mathcal{O},\mathcal{S})$
\State $(\hat{\mathcal{O}},\hat{\mathcal{S}}) \gets
       \textsc{AlignSizes}(\mathcal{O},\mathcal{S},\mathcal{P})$

\State \textcolor{gray}{// Layout Arrangement I: Collision Constraint}
\State $\varphi_{\text{layout}} \gets
       \textsc{Arrange}(\hat{\mathcal{O}},\hat{\mathcal{S}},\mathcal{P})$
\For{$t_1 = 1$ to $\text{maxTimeIter}$}
    \If{\textbf{not}\; $\textsc{CollisionFree}(\varphi_{\text{layout}})$}
        \State $\varphi_{\text{layout}} \gets \textsc{FixLayout}(\varphi_{\text{layout}},\textit{collision})$
    \Else
        \State \textbf{break} \Comment{collision‑free layout $\hat{\varphi}_{\text{layout}}$ found}
    \EndIf
\EndFor

\State \textcolor{gray}{// Layout Arrangement II: Reachability Constraint}
\For{$t_2 = 1$ to $\text{maxTimeIter}$}
    \If{\textbf{not}\; $\textsc{Reachable}(\hat{\varphi}_{\text{layout}})$}
        \State $\hat{\varphi}_{\text{layout}} \gets \textsc{FixLayout}(\hat{\varphi}_{\text{layout}},\textit{reachable})$
    \Else
        \State \textbf{break} \Comment{reachable layout $\varphi_{\text{layout}}^{\star}$ found}
    \EndIf
\EndFor

\State \textcolor{gray}{// Differentiable Scene Rendering}
\State $\mathcal{T} \gets \textsc{AnyReach}(\varphi_{\text{layout}}^{\star})$
\State $\mathbf{Scene}^{\star} \gets \textsc{ITFS}(\varphi_{\text{layout}}^{\star},\mathcal{T})$
\end{algorithmic}
\end{algorithm}

\subsection{Hierarchical LLM Agents Planning}
%\paragraph{High-level agent planning}
Given a concise user prompt \( T \), such as \textit{``A bedroom''}, our high-level planner adopts the reasoning capabilities of an LLM agent to semantically expand \( T \) and identify relevant object categories for the scene population. Select the appropriate types of objects that align with the scene style specified by the input prompt. The LLM agent also generates an indexed set $(O_i, S_i )$ for the room. Subsequently, the low-level LLM agent planner is used to enhance these assets with stylistic, textural, and material attributes. 

For spatial information, we first adopt Shap-E~\cite{shap-e}  to generate the corresponding point cloud representation  $\mathbf{p}_i=(x_i, y_i, z_i, c_i)$ for each object \(O_i\) according to the index $i$. We then predict the central position for each object by estimating candidate center coordinates $(x^{c}_i, y^{c}_i, z^{c}_i)$ in the scene. Each object $O_i$ is associated with a semantic label. To ensure semantic and physical plausibility, the physical agent aligns the real-world scale of each object and rescales it if inconsistencies are detected. The updated object parameters and spatial context $(\hat{O}_i, \hat{S}_i )$ are stored in \textit{.json} files for downstream tasks. Further details can be found in the Supplementary Material (Supp).


\subsection{Layout Arrangement Planning}
Taking the detail layout criterion $\varphi_{\text{layout}}=(\hat{O}_i, \hat{S}_i, \mathbf{p}_i)$ as input, we treat the indoor scene generation task as if in a closed space, following the same strategy used in a previous 3D layout arrangement method~\cite{holodeck2023}. The process begins with the construction of structural elements such as floors, walls, doors, and windows, followed by the arrangement of floor-mounted furniture and the placement of wall-mounted objects.
Next, we employ interactive optimization to update the layout design by verifying whether the generated layout satisfies our two constraints, which are specified as follows.

\paragraph{Collision Constraint} 
Given the inferred spatial constraints $\varphi_{\text{layout}}$ by LLM agents, we first adopt the depth-first-search algorithm to find a valid placement for object candidates inspired by Holodeck~\cite{holodeck2023}. We sequentially place objects according to the inferred symbolic rules, such as positioning objects close to walls, aligning them with other objects(~\eg~\textit{nightstands} beside a \textit{bed}), or oriented in specific directions. To enhance layout quality, we further decouple wall-mounted and ground-level object types while ensuring they both follow the same symbolic reasoning process.
Specifically, we define a collision-aware layout reward $\mathcal{R}_{\text{coll}}$ to ensure physical feasibility.

\begin{equation*}
\begin{aligned}
\mathcal{R}_{\text{coll}} =
- (\sum_{i \ne j} \text{IoU}_{3D}(b_i, b_j) + 
\sum_{i=1}^N \sum_{k=1}^{W} \text{IoU}_{3D}(b_i, \text{b}_k^{wall})),
\end{aligned}
\label{eq:coll_guide}
\end{equation*}
where $b_i$ and $b_j$ represent the bounding boxes of objects, and $b_k^{wall}$ denotes the bounding boxes of wall structures.
The $\text{IoU}_{3D}$ is a metric that measures the discrepancy between two candidate 3D bounding boxes. Note that a layout is valid only when $\mathcal{R}_{\text{coll}} = 0$. In practice, we set a time limit of 30 seconds for the $t_1$ iterating process; after this period, any objects that are still colliding will be removed.

\paragraph{Reachability Constraint} 
We ensure navigability by requiring all objects to be accessible to a virtual agent represented by the bounding box $b^{agent}$. Different from the reachability constraints in Physcene~\cite{physcene}, we rasterize the 3D Scene Map into a 2D traversable map and employ the A* search algorithm, initiating from a fixed starting point (~\eg~a doorway) to each object location. An object is considered reachable only if a valid path exists. The reachability reward $\mathcal{R}_{\text{reach}}$ is defined as follows:

\begin{equation*}
\mathcal{R}_{\text{reach}} = - \sum_{i=1}^{W} \text{IoU}_{3D}(b_i, b^{agent}).
\label{eq:agent_guide}
\end{equation*}
If an object is deemed unreachable, we undertake local spatial adjustments within a restricted search grid. Again, if no viable solution is identified in 30 seconds, the object will be removed from the layout. This integrated reasoning process ensures both physical plausibility and functional accessibility of the final layout $\varphi_{\text{layout}}^{\star}$.


\subsection{Differentiable Scene Optimization}
\paragraph{AnyReach Camera Trajectory Sampling}
Proir work AnyHome~\cite{anyhome} hypothesizes that the camera orients toward the room's center, generating egocentric trajectories that spiral around the scene. Meanwhile, they randomly sample the camera view to capture local details and refine object-level layouts. Unlike AnyHome, our AnyReach sampling strategy supports a more accurate ``Zoom-in and Zoom-out" approach to swiftly capture global and local views. 

Specifically, we utilize a spiral camera path across the upper hemisphere surrounding each object, with each camera directed toward the object's center. This spiral sampling aims to provide a global observation of the background and objects within the scene. When the ``Zoom-in" movement occurs, our camera employs the A* algorithm~\cite{Astar} to navigate to the object's location, ensuring the shortest path from the global view to the local object-level view. Taking advantage of A*, our approach conserves camera poses and minimizes the time spent observing irrelevant background such as \textit{wall} along the way. Once the camera reaches the object, we implement a ``Zoom-out" movement directly from the current object location to the original global path. This repeated jumping strategy prevents prolonged focus on a single object, ensuring comprehensive view supervision and reducing the object-level geometric blur from distant viewing. More visualization and implementation details are provided in the Supp.

%$\mathcal{T}$ explain 

%Moreover, our camera trajectory simulates how a robot or person observes the scene, providing a human-centered perspective for camera observation, which is beneficial for supporting navigation tasks and spatial understanding. 
%Moreover, A dense set of perimeter anchors is extracted from layout, and the shortest paths between these anchors and target objects are computed using the A* algorithm. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Interval Timestep Flow Sampling}  
In the rendering stage of~\cref{fig:pipeline}, to enhance the quality of raw 3D scene representations, we propose an Interval-Timestep Flow Sampling (ITFS) strategy that utilizes a range of different timesteps for generating 2D diffusion views. Our approach integrates ITFS with reflection flow matching and multi-timestep sampling, gradually optimizing scene quality from coarse to fine with enhancing semantic details (visualized in~\cref{fig:experiment_layout}).

Conditional Flow Matching (CFM)~\cite{lipman2023flow} has proven to be a robust framework for training continuous normalizing flows, primarily due to its efficiency in computation and overall effectiveness. To obtain higher-fidelity priors, we replace $\phi$ with Stable Diffusion 3.5~\cite{scaling}, which utilizes a rectified-flow formulation to model both the forward and reverse processes through a time-dependent vector field. The forward interpolation is defined as $x(t) = (1-t)\,x_0 + t\,\boldsymbol{\epsilon},~\boldsymbol{\epsilon}\sim\mathcal{N}(\mathbf{0},\mathbf{I})$, and the reverse field $v(x,t)=\tfrac{\partial x}{\partial t}$ is approximated by a neural network $v_{\phi}$. The training process adheres to the CFM objective:
\begin{equation*}
\mathcal{L}_\text{CFM}(\theta) = 
\mathbb{E}_{t, \boldsymbol{\epsilon}} \left[
    w(t) \left\|
        v_\phi(x_t; t) - (\boldsymbol{\epsilon} - x_0)
    \right\|_2^2
\right]
\end{equation*}

Building on the CFM objective function and SDS, we introduce a new \textbf{Flow Distillation Sampling (FDS)} strategy. The objective function $\nabla_{\theta}\mathcal{L}_\text{FDS}$ is defined as follows: 
\begin{equation*}
\label{eqn:x0-hatx0}
    \begin{aligned}
          \mathbb{E}_{t,\boldsymbol{\epsilon}}\Big[
          w(t)\bigl( v_\phi(x_t; y, t) -
          (\boldsymbol{\epsilon} - x_0) \bigr) \times \frac{\partial g(\theta, c)}{\partial \theta}
    \Big]
    \end{aligned}
\end{equation*}
Empirically, timesteps $t\in[200, 300]$ emphasize geometric features, while larger timesteps $t >500$ favor semantic alignment, a pattern also noted by DreamScene~\cite{dreamscene}. Since FDS samples in a single timestep, it cannot take advantage of both regimes. To address this limitation, we introduce ITFS which generates intermediate steps from small timestep intervals $t_0$ to large timestep intervals $t_m$. This is achieved during the optimization of the objective function  $\nabla_{\theta}\mathcal{L}_{\text{ITFS}}$:
 
\begin{equation*}
\label{eq:itfs}
    \begin{aligned}
    \mathbb{E}_{t,\boldsymbol{\epsilon}}\!\Bigg[
           \sum_{i=1}^{m} w(t_i)\,
           \bigl( v_\phi(x_t; y, t_i) - (\boldsymbol{\epsilon} - 
           x_0) \bigr) \times \frac{\partial g(\theta, c)}{\partial \theta}
         \Bigg] ,
    \end{aligned}
\end{equation*}
%\nabla_{\theta}\mathcal{L}_{\text{ITFS}}&=

where $m$ denotes the value of the sampling numbers. This multi-interval strategy allows early steps to refine geometric features while later steps consolidate semantic information. As a result, it produces 3D scenes that are both structurally accurate and visually coherent.





%\paragraph{Scene Rendering}
%Given the base point cloud representation, we first transform it into 3D Gaussians: $(\mathbf{x}_i,\mathbf{y}_i,\mathbf{z}_i, \mathbf{r}_i, \mathbf{s}_i, \mathbf{f}_i)$ for each object $O_i$, where \(\mathbf{x}_i,\mathbf{y}_i,\mathbf{z}_i \in \mathbb{R}^3\) denotes the position, \(\mathbf{r}_i \in \mathrm{SO}(3)\) the rotation, \(\mathbf{s}_i \in \mathbb{R}^3\) the scale, and \(\mathbf{f}_i \in \mathbb{R}^c\) the feature embedding. %The room scene is formally represented as  \( \varphi_{\text{layout}}^{\star} = \{(O_i, S_i)\}_{i=1}^N \), where each \( O_i \) corresponds to a distinct object modeled via 3DGS.

==> history/sec/4_experiments.tex <==
\begin{table*}[t!]  
\centering
\setlength{\tabcolsep}{1.4mm}
\small % 9pt
%\begin{tabular}{c|c|ccccccc}
\begin{tabular}{c|c|c c c c c c c}
        \toprule
        Type &  Method & \shortstack{Layout \\ Planning}  & \shortstack{End-to-End \\ Generation} & \shortstack{Room \\ Scene} & \shortstack{Edition} & \shortstack{Realistic \\ (object)} & \shortstack{Realistic \\ (scene)} & \shortstack{Surface \\ Reconstruction} \\
        \midrule
        
        \multirow{4}{*}{Visual-Guided} 
        & Text2Room~\cite{Text2Room} & - & - & - & - & \ding{51} & \ding{51} & \ding{51} \\
        & SceneWiz3D~\cite{Zhang_2024_CVPR} & - & - & - & \ding{51} & -  & - & \ding{51} \\
        & Pano2Room~\cite{pu2024pano2room} & - & - & - & \ding{51} & -  & - & \ding{51} \\
        & Director3d~\cite{director3d} & - & - & - & \ding{51} & -  & - & \ding{51} \\
        & Scene4U~\cite{scene4u} & - & - & \ding{51} & - & -  & - & \ding{51} \\
        \midrule

        \multirow{6}{*}{Rule-based} 
        & Set-the-Scene~\cite{setthescene} & \ding{51} & - & - & - & \ding{51} & \ding{51} & \ding{51} \\
        & GALA3D~\cite{GALA3D} & \ding{51} & \ding{51} & - & \ding{51} & \ding{51} & -& - \\
        & AnyHome~\cite{anyhome} & \ding{51} & - & \ding{51} & \ding{51} & \ding{51} & -  & \ding{51} \\
        & GraphDreamer~\cite{graphdreamer} & \ding{51} & \ding{51} & - & \ding{51} & \ding{51} & -  & - \\
        & DreamScene~\cite{dreamscene} & \ding{51} & \ding{51} & - & \ding{51} & \ding{51} & \ding{51}& - \\
        
        % & Ours & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
        \midrule
        \rowcolor{lightgray!30}
        & Ours & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of 3D indoor scene synthesis methods, categorized into rule-based and visual-guided approaches. \ding{51} means capability supported; `-' means without that capability. Our method demonstrates comprehensive capabilities across all metrics.}
\label{tab:dataset-table}
\end{table*}

\begin{figure*}[t!]
  \centering
  \includegraphics[width=1.0\textwidth]{figures/demo_show.pdf}
  \caption{We compare the interactive scene 3D generation with Set-the-Scene~\cite{setthescene}, GALA3D~\cite{GALA3D} and DreamScene~\cite{dreamscene}.}
  \label{fig:experiments}
\end{figure*}

\section{Experiments}
\label{experiments}
\paragraph{Implementation Details}
We utilize GPT-4~\cite{gpt4} as our LLM agents for both reasoning and grounding modules. Shap-E~\cite{shap-e} generated point clouds serve as the initial representation of objects, while Stable Diffusion 3.5 Medium~\cite{StabilityAI23} provides guidance for rendering 3D scene models. We set the rendering iterations to 1500 and the resolution to 512 $\times$ 512, and ITFS sampling interval value $m=3$, drawing $t_0\!\sim\![200,400]$, $t_1\!\sim\![400,600]$ and $t_2\!\sim\![600,800]$.  We tested~\Ourmodel~and all baselines on the same NVIDIA 4090 GPU for fair comparison.

%=================Qualitative Results=================
\subsection{Qualitative Results}
\cref{fig:experiments} compares our model with other state-of-the-art methods. We observe that GALA3D~\cite{GALA3D} lacks adequate asset diversity, while Set-the-Scene~\cite{setthescene} shows geometric discontinuities. Additionally, DreamScene~\cite{dreamscene} suffers from particle opacity artifacts and coarse surface geometry, all of which compromise visual fidelity. In contrast, our model generates physically plausible scene synthesis. The decoupled guidance and layout arrangement approaches ensure physical interaction constraints without sacrificing scene diversity. As a result, our model can produce high-quality 3D scenes with object-level decoupling, surpassing prior differentiable approaches in rendering speed, visual quality, and geometric consistency, all while maintaining editability.

\paragraph{Effectiveness of ITFS}
As illustrated in \cref{fig:experiment_layout}, our method leverages implicit layout knowledge obtained from a 2D generation model to further optimize the 3D scene. The proposed ITFS strategy significantly enhances scene generation by refining object orientation and detail. The coach labels in the two yellow boxes guide the orientation to achieve a more rational and coherent perspective. As the timesteps progress from $m = 0$ to $m = 3$, the scene quality is optimized from a coarse representation to a fine, detailed depiction. This progression not only improves geometric accuracy but also enriches the semantic details, resulting in a more realistic and contextually appropriate rendering.

%presents the ITFS output used as the observation input, and (b) shows the pseudo-GT produced by the 2D diffusion model. The lower row illustrates the trade-off between pseudo-GT quality and training time across varying ITFS sampling intervals
%We take the rendered view as input to  is processed through 2D diffusion to produce a pseudo-GT view in~\cref{fig:experiment_layout} (b), featuring a corrected sofa orientation that guides layout adjustments. Given that such edits can significantly influence the convergence rate of differentiable models, we carefully regulate their intensity by adjusting the number of ITFS acquisitions and the sampling interval, as shown in the last two rows of \ref{fig:experiment_layout}. This approach effectively balances correction quality with computational cost.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth, height=0.40\textwidth]{figures/experiment_layout.png}
  \caption{Effectiveness of ITFS. The coach labels in yellow boxes guide the orientation towards a more rational perspective. As the timesteps progress from $m = 0$ to $m = 3$, the scene quality is optimized from a coarse representation to a fine depiction, enriched with more semantic details.}
  \label{fig:experiment_layout}
\end{figure}

%=================
\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{1.3mm}
    \small 
    \begin{tabular}{l|ccccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{User Study} & \multicolumn{3}{c}{Quality} \\
        \cmidrule{2-6}
        & $\uparrow$ Rationality & $\uparrow$ Quality & $\uparrow$ AS & $\uparrow$ IR  & $\uparrow$ CS $_{\%}$ \\
        \midrule
        Set-the-scene & 1.13 & 2.80 & 4.83 & 41.10 & 26.05 \\
        GALA3D & 2.61 & 3.22 & 5.07 & 42.67 & 25.40 \\
        DreamScene & 3.10 & 3.15 & 5.13 & 43.85 & 26.77 \\
        \textbf{Ours} & \textbf{4.10} & \textbf{3.86} & \textbf{5.31} & \textbf{48.83} & \textbf{28.44} \\
        \bottomrule
    \end{tabular}
    % \caption{Quantitative (AS is Aesthe. Score~\cite{ava}, IR is ImageReward(T3Bench)~\cite{imagereward} and CS is CLIP Score~\cite{clipscore}) and user study results on the Indoor Scene Generation task. Our method consistently outperforms baselines across all evaluation metrics.}
    \caption{Quantitative evaluation across open soucre method on Indoor Scene Generation. Our method demonstrates consistent superiority across quality metrics (Rationality, Quality) and user study metrics (AS, IR, CS).}
    \label{tab:text_3d_campare}
\end{table}

\subsection{Quantitative Results}
\paragraph{User Study for Semantic Alignment} 
We conducted a user study to compare our approach with existing open source methods, focusing on scene quality and scene authenticity. We selected five common indoor scenes,~\ie~living room, kitchen, dining room, bedroom, and workplace, for quantitative evaluation. Thirty participants, including professional interior designers, Embodied-AI algorithm engineers, and graduate students, evaluated these scenes on a 1-to-5 scale, indicating their satisfaction from low to high. As shown in~\cref{tab:text_3d_campare}, our method achieved the highest scores across different downstream fields.

\paragraph{3D Scene Generation Quality}
As shown in~\cref{tab:text_3d_campare}, we tested our approach on three qualitative metrics. Aesthe. Score (AS)~\cite{ava} that evaluates aesthetic quality of scene. We also compared 3D generation quality on the ImageReward (T3Bench) (IR)~\cite{imagereward}, which refers to image reward applicantion in T3Bench, and CLIP Score (CS)~\cite{clipscore} to evaluation the text-3D scene alignment. Set-the-Scene~\cite{setthescene}, GALA3D~\cite{GALA3D} and DreamScene~\cite{dreamscene} both lack of scene diversity and rendering realism issues, bringing negatively increasing their overall scores. Our method performs well on all metrics, which is consistent with the results shown in the user study, which once again proves the superiority of our paradigm combining LLM, scene plan and ITFS generation.


==> history/sec/5_conclusion.tex <==
\section{Conclusion}
We present~\Ourmodel, an automatic framework for text-to-3D scene generation. Following a pipeline of ‘Reasoning-Grounding, Arrangement, and Optimization,’ our method enhances diversity, complexity, and efficiency for text-to-3D scene generation. By integrating LLMs for scene layout guidance, collision and reachability constraints for layout arrangement, and specific sampling strategies for rendering, our method generates explicit layout criteria to guide rational spatial placements. Experimental results demonstrate that~\Ourmodel~outperforms existing methods in generating diverse and complex scenes while requiring fewer computational resources for realistic 3D representation. %Extensive experiments assess scene quality, semantic alignment, and layout rationality, demonstrating the practical benefits of our approach.

\paragraph{Limitation}
Despite its computational efficiency, our method operates on an RTX 4090 GPU with 24GB VRAM. To balance efficiency and performance within this memory constraint, we limit the increase in the number of 3D Gaussians during later optimization stages. This results in insufficient resources to adequately model the fine-grained scattering behavior of light on complex materials and structures. Future work will focus on enhancing visual realism by addressing these limitations, particularly in improving the modeling of complex light transport and recovering finer geometric details, to generate scenes suitable for a broader range of demanding applications.

%inherits limitations from its dependence on a pre-trained 2D image diffusion model, which lacks prior specialized knowledge on the visual fidelity of real-world scenes. Additionally

==> history/sec/preliminary.tex <==
\section{Preliminary}

\paragraph{3D Layout Arrangement}
%It generates 3D instance properties stored in an unordered object set and retrieves the most similar geometry for each object configuration, which is characterized as a concatenation of different attributes, including location, size, orientation, semantics, and geometry features.

Taking layout descriptions as input, this problem aims to arrange unordered 3D assets from existing datasets within a 3D environment. Formally, given a layout criterion \( \varphi_{\text{layout}} \), a space defined by four walls oriented along the cardinal directions $\{w_1, \dots, w_4\}$, and a set of \( N \) 3D meshes $\{m_1, \dots, m_N\}$, the objective is to create a 3D scene that reflects the most accurate spacial relationships of the provided layout configuration. Previous methods~\cite{holodeck2023,feng2023layoutgpt,Sun_2025_CVPR} treat indoor layout as 3D reasoning tasks, arranging objects in space according to open-ended language instructions. They assume that the input 3D objects are upright and an off-the-shelf vision-language model (VLM),~\eg~GPT-4~\cite{gpt4}, to determine the front-facing orientations of the objects. As one of the representative methods, LayoutVLM~\cite{Sun_2025_CVPR} annotates each object with a concise textual description \( s_i \), and the dimensions of its axis-aligned bounding box, after rotating to face the \( +x \), are represented as \( b_i \in \mathbb{R}^3 \). The desired output of the layout generation process is the pose of each object \(p_i = (x_i, y_i, z_i, \theta_i)\), which includes 3D position and its rotation about the \( z \)-axis.

\paragraph{Neural Representation} 
Unlike explicit representations such as meshes or point clouds, implicit neural representation methods train a 3D model through differentiable rendering. There are mainly two types of neural representations: Neural Radiance Fields~\cite{nerf} and 3D Gaussian Splatting(3DGS)~\cite{3DGS}. 3DGS represents the scene as a set of 3D Gaussians $\{\mathcal{G}_{i}\}_{i=1}^{M}$, each parametrized with center position $\mathbf{\mu}_i \in \mathbb{R}^{3}$, covariance $\mathbf{\Sigma}_i \in \mathbb{R}^{3\times 3}$, color $c_i \in \mathbb{R}^{3}$, and opacity $\alpha_i \in \mathbb{R}^{1}$. The 3D Gaussians can be queried by $\mathcal{G}(x)~= e^{-\frac{1}{2}(x)^{T}\Sigma^{-1}(x)}$, where $x$ represents the distance between $\mathbf{\mu}$ and the query point. The 3D Gaussians are optimized through differentiable rasterization for projection rendering, comparing the resulting image to the training views in the captured dataset using image loss metrics. In the text-to-3D task, there is typically no ground truth (GT) image available. Existing works usually employ a diffusion model to generate pseudo-GT images for distilling the 3D representation.
% To render a projection image and compute the color of each pixel, a neural point-based rendering approach is used. A ray $r$ is cast from the camera center, calculating accumulated color $c_i$ of intersected 3D Gaussians  density $\sigma_{i}$ along the ray:
% $C(r) = \sum_{i \in \mathcal{N}}
% 	c_{i}\sigma_{i}
% 	\prod_{j=1}^{i-1}(1-\sigma_{j}), 
%         \sigma_{i} = \alpha_{i} \mathcal{G}(x_i)$
% where $\mathcal{N}$ represents the number of sample points on ray $r$. 
%,$c_{i}$ and $\alpha_{i}$ denote the color and opacity of the i-th Gaussian, and $x_i$ is the distance between the point and the i-th Gaussian. It develops differentiable rasterization for projection rendering and optimizes Gaussians via image losses

\paragraph{Diffusion Models}
Diffusion models~\cite{diffusion,ddim} generate data by iteratively denoising a sample from pure noise.  During training, a noisy version of a data sample $\mathbf{x} \sim p_{\text{data}}$ is generated as $\mathbf{x}_{t} = \sqrt{\bar{\alpha}_{t}}\,\mathbf{x} + \sqrt{1 - \bar{\alpha}_{t}}\bm{\epsilon}$, where $\bm{\epsilon} \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ is standard Gaussian noise, and $\bar{\alpha}_{t}$ controls noise level. The discrete diffusion timestep $t$ is sampled from a uniform distribution $p_t \sim \mathcal{U}(0, t_{max})$. The denoising network $\theta$ predicts the added noise $\bm{\epsilon}_{\theta}$ and is optimized with the score matching objective:
$\mathcal{L}_t=\mathbb{E}_{\mathbf{x}\sim p_{\text{data}},\, t \sim p_t,\, \bm{\epsilon}\sim \mathcal{N}(\mathbf{0}, \mathbf{I})}\left[\left\lVert \bm{\epsilon} - \bm{\epsilon}_{\theta}(\mathbf{x}_{t}, t)\right\rVert_2^2\right]$.

DreamFusion~\cite{dreamfusion} distills 3D representations from a 2D text-to-image diffusion model through Score Distillation Sampling (SDS). Let $\theta$ denote the parameters of a differentiable 3D representation, and let $g$ represent a rendering function. The rendered image produced for a given camera pose $c$ can be expressed as $x_0 = g(\theta, c)$, where $x_0$ is the clean (noise-free) rendering.  A noisy view at timestep $t$ is obtained as: $ x_t = \alpha_t\,x_0 + \sigma_t\,\boldsymbol{\epsilon}.$
Then SDS distills $\theta$ through a 2D diffusion model $\phi$ with frozen parameters as follows:
\begin{equation*}
\label{eqn:sds}
    \begin{aligned}
    \nabla_{\theta} \mathcal{L}_\text{SDS}(\theta) = 
    \mathbb{E}_{t, \boldsymbol{\epsilon}, c} 
    \Bigg[ 
        & w(t) \left( \boldsymbol{\epsilon}_\phi(\mathbf{x}_t; y, t) 
        - \boldsymbol{\epsilon} \right)
        \times \frac{\partial g(\mathbf{\theta}, c)}{\partial \theta}
    \Bigg], 
    \end{aligned}
\end{equation*}
where $w(t)$ is a timestep-dependent weight and $\boldsymbol{\epsilon}_{\phi}$ is the noise estimator of the frozen diffusion model~$\phi$ conditioned on the text prompt $y$.

%\boldsymbol{\epsilon}\sim\mathcal{N}(\mathbf{0},\mathbf{I})

==> history/table1.tex <==
\begin{table*}
\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
\multirow{1}{*}{Methods} 
& Time $\downarrow$  & Single obj. $\uparrow$ & Single w/surr. $\uparrow$ & Multi obj. $\uparrow$ & $\mathbf{Average}_{\text{}}$ $\uparrow$  \\ 
\midrule
SJC~\cite{Lu23SJC}& -- & 24.7 & 19.8 &  11.7 &18.7  \\
DreamFusion~\cite{Poole22} &6 hours & 24.4&  24.6   & 16.1 & 21.7   \\
Fantasia3D~\cite{Chen23Fantasia} &6 hours & 26.4&  27.0   & 18.5 & 24.0  \\
LatentNeRF~\cite{Metzer22Latent} &15 minutes & 33.1&  30.6   & 20.6 &28.1  \\
Magic3D~\cite{Lin23Magic3D} &5.3 hours & 37.0 &  35.4   & 25.7 &32.7  \\
ProlificDreamer~\cite{Wang23Prolific} &10 hours & 49.4&  44.8  & 35.8 & 43.3  \\
\midrule
RoomDreamer (Ours) &  \textbf{7 minutes} & \textbf{58.3}  & \textbf{55.4}  & \textbf{47.8}& \textbf{53.8}  \\
\bottomrule
\end{tabular}
}
\caption{
    \textbf{Quantitative comparison on text-driven scene generation.} 
    % We compare with ATISS and Diffuscene on common perceptual quality scores FID, SCA, CKL, as well as physical plausibility measured in collision rate $\mathbf{Col}$.
    }
    \label{tab:Unconditioned Scene Synthesis}
\end{table*}

% \multirow{7}{*}{Method} & \multicolumn{5}{c}{Bedroom} & \multicolumn{5}{c}{Living Room} & \multicolumn{5}{c}{Dining Room} \\ \cmidrule(r){2-6} \cmidrule(r){7-11} \cmidrule(r){12-16} 
% & FID $\downarrow$  & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$ & $\mathbf{Col}_{\text{scene}}$ $\downarrow$ & FID $\downarrow$  & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$ & $\mathbf{Col}_{\text{scene}}$ $\downarrow$ & FID $\downarrow$ & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$  & $\mathbf{Col}_{\text{scene}}$ $\downarrow$  \\ 
% \midrule
% SJC~\cite{paschalidou2021atiss}&36.92& \textbf{49.24} &0.0036&  0.255 & 0.50& 55.76& 53.33 & 0.0016 &   0.372 & 0.870 &41.89 & 58.20 & 0.0028 & 0.483 & 0.91 \\
% DreamFusion~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
% Fantasia3D~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
% LatentNeRF~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
% Magic3D~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
% ProlificDreamer~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
% \midrule
% RoomDreamer (Ours) &  \textbf{28.56} & 55.71  & \textbf{0.0030}  & \textbf{0.187}& \textbf{0.35}  & \textbf{40.67}   &  56.20   &  0.0015  & \textbf{0.130}    & \textbf{0.477}  &   37.88   &    58.74  & \textbf{ 0.0022}    & \textbf{0.134}    &  \textbf{0.40}\\
% \bottomrule
% \end{tabular}
% }
% \caption{
%     \textbf{Quantitative comparison on text-driven scene generation.} 
%     % We compare with ATISS and Diffuscene on common perceptual quality scores FID, SCA, CKL, as well as physical plausibility measured in collision rate $\mathbf{Col}$.
%     }
%     \label{tab:Unconditioned Scene Synthesis}
% \end{table*}

==> history/table2.tex <==
\begin{table*}
\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccccc}
\toprule
\multirow{7}{*}{Method} & \multicolumn{5}{c}{Bedroom} & \multicolumn{5}{c}{Living Room} & \multicolumn{5}{c}{Dining Room} \\ \cmidrule(r){2-6} \cmidrule(r){7-11} \cmidrule(r){12-16} 
& FID $\downarrow$  & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$ & $\mathbf{Col}_{\text{scene}}$ $\downarrow$ & FID $\downarrow$  & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$ & $\mathbf{Col}_{\text{scene}}$ $\downarrow$ & FID $\downarrow$ & SCA $\downarrow$ & CKL $\downarrow$ & $\mathbf{Col}_{\text{obj}}$ $\downarrow$  & $\mathbf{Col}_{\text{scene}}$ $\downarrow$  \\ 
\midrule
SJC~\cite{paschalidou2021atiss}&36.92& \textbf{49.24} &0.0036&  0.255 & 0.50& 55.76& 53.33 & 0.0016 &   0.372 & 0.870 &41.89 & 58.20 & 0.0028 & 0.483 & 0.91 \\
DreamFusion~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
Fantasia3D~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
LatentNeRF~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
Magic3D~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
ProlificDreamer~\cite{tang2023diffuscene} &28.63 & 51.33&  0.0031   & 0.238  & 0.42 & 54.36& \textbf{50.24} & \textbf{0.0010}&  0.183  & 0.570 &  \textbf{37.68} & \textbf{57.60}    &  0.0031 &  0.253 & 0.63 \\
\midrule
RoomDreamer (Ours) &  \textbf{28.56} & 55.71  & \textbf{0.0030}  & \textbf{0.187}& \textbf{0.35}  & \textbf{40.67}   &  56.20   &  0.0015  & \textbf{0.130}    & \textbf{0.477}  &   37.88   &    58.74  & \textbf{ 0.0022}    & \textbf{0.134}    &  \textbf{0.40}\\
\bottomrule
\end{tabular}
}
\caption{
    \textbf{User Study.} 
    % We compare with ATISS and Diffuscene on common perceptual quality scores FID, SCA, CKL, as well as physical plausibility measured in collision rate $\mathbf{Col}$.
    }
    \label{tab:Unconditioned Scene Synthesis}
\end{table*}

==> preamble.tex <==
% 
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


